OLMoASR: Open Models and Data for Training Robust Speech Recognition Models

Improvements in training data scale and quality have led to significant advances, yet its influence in speech recognition remains underexplored. In this paper, we present a large-scale dataset, OLMoASR-Pool, and series of models, OLMoASR, to study and develop robust zero-shot speech recognition models. Beginning from OLMoASR-Pool, a collection of 3M hours of English audio and 17M transcripts, we design text heuristic filters to remove low-quality or mistranscribed data. Our curation pipeline produces a new dataset containing 1M hours of high-quality audio-transcript pairs, which we call OLMoASR-Mix. We use OLMoASR-Mix to train the OLMoASR-Mix suite of models, ranging from 39M (tiny.en) to 1.5B (large.en) parameters. Across all model scales, OLMoASR achieves comparable average performance to OpenAI's Whisper on short and long-form speech recognition benchmarks. Notably, OLMoASR-medium.en attains a 12.8\% and 11.0\% word error rate (WER) that is on par with Whisper's largest English-only model Whisper-medium.en's 12.4\% and 10.5\% WER for short and long-form recognition respectively (at equivalent parameter count). OLMoASR-Pool, OLMoASR models, and filtering, training and evaluation code will be made publicly available to further research on robust speech processing.

==> components/sections/data/curation/dedupcont.tex <==
\subsubsection{Decontamination and deduplication} \label{sec:declean}
We performed transcript level fuzzy deduplication using minhash. We used the parameters from FineWeb \citep{penedo2024finewebdatasetsdecantingweb}, where we used 5-grams of tokens and computed 112 hash functions, split into 14 buckets of 8 hashes each. If any pair of transcripts has the same 8 hashes in any one bucket, they are marked as duplicates. This procedure targets documents that have a Jaccard similarity of 75\%. We performed this on 17M total transcripts and removed 505K transcripts for a total deduplication removal rate of 3\%.
Decontamination was performed by a simple n-gram search. In particular, we decontaminate the evaluation datasets of TED-LIUM3 against our training corpus. First we collect all n-grams of size 10 from the evaluation dataset and check for their presence in each training dataset transcript. If any n-gram is present, we mark the training document as contaminated and do not include it in our training sets. We apply this procedure to 17M transcripts and find only 286 contaminated transcripts.
